Domain Generalization via Selective Consistency Regularization for Time Series Classification

Domain generalization methods aim to learn models robust to domain shift with data from a limited number of source domains and without access to target domain samples during training. Popular domain alignment methods for domain generalization seek to extract domain-invariant features by minimizing the discrepancy between feature distributions across all domains, disregarding inter-domain relationships. In this paper, we instead propose a novel representation learning methodology that selectively enforces prediction consistency between source domains estimated to be closely-related. Specifically, we hypothesize that domains share different class-informative representations, so instead of aligning all domains which can cause negative transfer, we only regularize the discrepancy between closely-related domains. We apply our method to time-series classification tasks and conduct comprehensive experiments on three public real-world datasets. Our method significantly improves over the baseline and achieves better or competitive performance in comparison with state-of-the-art methods in terms of both accuracy and model calibration.

==> sections/background.tex <==
\section{Background}
\label{sec: background}

\subsection{Generalization Bound on Target Risk}
\label{sec: bound}

In multi-source DA, the target domain risk is bounded by a sum consisting empirical source domain risks and divergence between source and target domains, as stated in Theorem~\ref{theorem: DA}

\begin{theorem}~\cite{Zhao2018AdversarialMS}
Let $\mathcal{H}$ be a hypothesis class with VC dimension $v$. For source domain $\{\hat{S}_m\}_{m=1}^M$ with $\frac{N}{M}$ i.i.d. samples from each domain, and target domain $\hat{T}$ with $N$ samples, with probability $1-\delta$, for all $\gamma \in \mathcal{H}$ and $\forall a \in \mathbb{R}^M_+$ such that $\sum_{m=1}^M a_m = 1$,
\begin{align}
    \epsilon_T(\gamma) \leq 
    & \sum_{m=1}^M a_i \left( \hat{\epsilon}_{S_m}(\gamma) + \frac{1}{2}div_{\mathcal{H}}(\hat{T}; {\hat{S}_m}) \right) +
    r_a \nonumber \\ 
    & + O\left( \sqrt{ \frac{1}{N} \left( \log\frac{1}{\delta} + v\log\frac{N}{v} \right) } \right) \label{eqn: task_risk_bound}
\end{align}
where 
$\epsilon(\gamma)$ and $\hat{\epsilon}(\gamma)$ are risk and empirical risk of $\gamma$ w.r.t. the true labeling function respectively,
$r_a$ is upper bound of $\text{inf}_{\gamma \in \mathcal{H}} \left( \sum_{m=1}^M a_m \epsilon_{S_m}(\gamma) + \epsilon_{T}(\gamma) \right)$, and $\mathcal{H}$-divergence $div_\mathcal{H}(T; S) \defeq 2\text{sup}_{A \in \mathcal{A}_\mathcal{H}} \| P_T(A) - P_S(A)\|$ with $A_\mathcal{H} \defeq \{\gamma^{-1}(\{1\}) | \gamma \in \mathcal{H}\}$. \label{theorem: DA}
\end{theorem}

In DA, adversarial learning and regularization are used to align source and target domains to directly reduce $\mathcal{H}$-divergence.
Unlike DA, target domain $\hat{T}$ is unavailable during training for DG. Aligning source domains helps to prevent learning spurious features, but aligning all source domains does not guarantee reducing $\mathcal{H}$-divergence, and may decrease feature diversity which in turn increases $\mathcal{H}$-divergence.

\textbf{Analysis of bound terms:}
We create a two-channel toy dataset for binary classification of sawtooth and square-shaped signals to compare bound terms in Equation~\ref{eqn: task_risk_bound} and empirical target risk.
Domain A and B have shape signals on channel 1. Domain C and D additionally have square signals on channel 2 for the square signal class. Noise added to signal is Gaussian distributed with standard deviation 2 for A and B and 4 for C and D. We use D as target and the rest as source.

We implement our proposed method with regularization on domain A and B.
In Table~\ref{tab:target_risk}, lower $\mathcal{H}$-divergence indicates lower target risk. Our proposed method has lower $\mathcal{H}$-divergence and target risk than DANN-DG and CDANN-DG. By not aligning domain C, we also allow the model to retain channel 2 signal features which target domain D can use for classification. More details are in Appendix B.
\input{tables/target_risk}
